Graphical Contrastive Losses for Scene Graph Parsing

Most scene graph parsers use a two-stage pipeline to detect visual relationships: the first stage detects entities, and the second predicts the predicate for each entity pair using a softmax distribution. We find that such pipelines, trained with only a cross entropy loss over predicate classes, suffer from two common errors. The first, Entity Instance Confusion, occurs when the model confuses multiple instances of the same type of entity (e.g. multiple cups). The second, Proximal Relationship Ambiguity, arises when multiple subject-predicate-object triplets appear in close proximity with the same predicate, and the model struggles to infer the correct subject-object pairings (e.g. mis-pairing musicians and their instruments). We propose a set of contrastive loss formulations that specifically target these types of errors within the scene graph parsing problem, collectively termed the Graphical Contrastive Losses. These losses explicitly force the model to disambiguate related and unrelated instances through margin constraints specific to each type of confusion. We further construct a relationship detector, called RelDN, using the aforementioned pipeline to demonstrate the efficacy of our proposed losses. Our model outperforms the winning method of the OpenImages Relationship Detection Challenge by 4.7\% (16.5\% relative) on the test set. We also show improved results over the best previous methods on the Visual Genome and Visual Relationship Detection datasets.

==> tex/fig/fig_examples.tex <==
\begin{figure*}[t!]
  \centering
  \begin{subfigure}{2.1\columnwidth}
    \centering
    \begin{subfigure}{0.32\columnwidth}
      \centering
      \includegraphics[width=\textwidth]{fig/1c1af13a505c2808_gt.JPG}
    % \caption{ground truth}
    % \label{fig:gt}
    \end{subfigure}
    \centering
    \begin{subfigure}{0.32\columnwidth}
      \centering
      \includegraphics[width=\textwidth]{fig/1c1af13a505c2808_wrong_marked.JPG}
    % \caption{conv\_body\_det}
    % \label{fig:det_conv}
    \end{subfigure}
    \centering
    \begin{subfigure}{0.32\columnwidth}
      \centering
      \includegraphics[width=\textwidth]{fig/1c1af13a505c2808_right_marked.JPG}
    % \caption{conv\_body\_rel}
    % \label{fig:prd_conv}
    \end{subfigure}
  \end{subfigure}
  
  \centering
  \begin{subfigure}{2.1\columnwidth}
    \centering
    \begin{subfigure}{0.32\columnwidth}
      \centering
      \includegraphics[width=\textwidth]{fig/6935bb10af767315_gt.JPG}
    % \caption{ground truth}
    % \label{fig:gt}
    \end{subfigure}
    \centering
    \begin{subfigure}{0.32\columnwidth}
      \centering
      \includegraphics[width=0.99\textwidth]{fig/6935bb10af767315_wrong_marked.JPG}
    % \caption{conv\_body\_det}
    % \label{fig:det_conv}
    \end{subfigure}
    \centering
    \begin{subfigure}{0.32\columnwidth}
      \centering
      \includegraphics[width=0.99\textwidth]{fig/6935bb10af767315_right_marked.JPG}
    % \caption{conv\_body\_rel}
    % \label{fig:prd_conv}
    \end{subfigure}
  \end{subfigure}
  
%   \centering
%   \begin{subfigure}{2.1\columnwidth}
%     \centering
%     \begin{subfigure}{0.32\columnwidth}
%       \centering
%       \includegraphics[width=\textwidth]{fig/c959dc327f67679a_gt.JPG}
%     \end{subfigure}
%     \centering
%     \begin{subfigure}{0.32\columnwidth}
%       \centering
%       \includegraphics[width=0.99\textwidth]{fig/c959dc327f67679a_wrong_marked.JPG}
%     \end{subfigure}
%     \centering
%     \begin{subfigure}{0.32\columnwidth}
%       \centering
%       \includegraphics[width=0.99\textwidth]{fig/c959dc327f67679a_right_marked.JPG}
%     \end{subfigure}
%   \end{subfigure}
  
  \centering
  \begin{subfigure}{2.1\columnwidth}
    \centering
    \begin{subfigure}{0.32\columnwidth}
      \centering
      \includegraphics[width=\textwidth]{fig/d95cf3f7f415b434_gt.JPG}
    \caption{ground truth}
    \label{fig:gt}
    \end{subfigure}
    \centering
    \begin{subfigure}{0.32\columnwidth}
      \centering
      \includegraphics[width=0.99\textwidth]{fig/d95cf3f7f415b434_wrong_marked.JPG}
    \caption{$L_0$ only}
    \label{fig:det_conv}
    \end{subfigure}
    \centering
    \begin{subfigure}{0.32\columnwidth}
      \centering
      \includegraphics[width=0.99\textwidth]{fig/d95cf3f7f415b434_right_marked.JPG}
    \caption{all losses}
    \label{fig:prd_conv}
    \end{subfigure}
  \end{subfigure}
\setlength\belowcaptionskip{-2ex}
\captionsetup{font=small}
\caption{Example images where RelDN with only $L_0$ predicts incorrectly while our loss succeeds. For each image we check the number of its ground truth relationships, then we output the same number of top predictions from a model to see its ranking accuracy. Red boxes in (b) highlight the false predictions from RelDN with $L_0$ only and green boxes in (c) highlight the correct ones from RelDN with all losses.}
\label{fig:examples}
\end{figure*}

==> tex/fig/fig_fpn_rel.tex <==
\begin{figure}[t]
  \centering
  \includegraphics[width=0.9\columnwidth]{fig/FPN_rel_pyramid.pdf}
  \captionsetup{font=small}
  \setlength\belowcaptionskip{-2ex}
  \caption{The lateral connections for predicate CNN features. P2-P5 are fixed and used as entity detector features, while Q2-Q5 are predicate features, which are trained to transform entity features to features for predicates.}
  \label{fig:fpn_rel}
\end{figure}

==> tex/fig/fig_losses.tex <==
\begin{figure*}[t!]
  \centering
  \begin{subfigure}{0.34\columnwidth}
    \centering
    \begin{subfigure}{0.9\columnwidth}
      \centering
        \includegraphics[width=\textwidth]{fig/class_agnostic}
    \end{subfigure}
%   \captionsetup{font=small}
  \caption{class agnostic loss}
  \label{fig:class_agnostic}
  \end{subfigure}
  \centering
  \begin{subfigure}{0.83\columnwidth}
    \centering
    \begin{subfigure}{0.95\columnwidth}
      \centering
        \includegraphics[width=\textwidth]{fig/o_class_aware}
    \end{subfigure}
%   \captionsetup{font=small}
  \caption{entity class aware loss}
  \label{fig:o_class_aware}
  \end{subfigure}
  \centering
  \begin{subfigure}{0.83\columnwidth}
    \centering
    \begin{subfigure}{0.97\columnwidth}
      \centering
        \includegraphics[width=\textwidth]{fig/p_class_aware}
    \end{subfigure}
%   \captionsetup{font=small}
  \caption{predicate class aware loss}
  \label{fig:p_class_aware}
  \end{subfigure}
\setlength\belowcaptionskip{-2ex}
\captionsetup{font=small}
\caption{Illustrations of the three losses. Squares, circles and lines represent $s, p, o$, respectively. Note: \textit{light blue} and \textit{light red} mean that we only care about positiveness but not the class of that node or edge, \eg, the \textit{light blue} circles in (a) represent positive entities regardless of their specific classes, and \textit{light red} lines in (b) represent negative (non-related) $so$ pairs regardless of their predicates. \textit{Green} and \textit{purple} represent two specific example classes, \eg, \textit{purple} circles in (b) or \textit{purple} lines in (c) belong to one entity or predicate class while \textit{green} ones belong to another.}
\label{fig:losses}
\end{figure*}

==> tex/tab/tab_abl_prd.tex <==
\begin{table}[t!]
\centering
\resizebox{0.8\columnwidth}{!}{
\begin{tabular}{c | c c c c}
\hline
 & R@50 & wmAP$_{rel}$ & wmAP$_{phr}$ & score$_{wtd}$ \\
\hline
\hline
ImageNet init & 74.82 & 34.93 & 37.96 & 44.12 \\
entity detector & 74.85 & 35.06 & 38.15 & 44.25 \\
% obj transform & \textbf{75.03} & 35.21 & 38.12 & 44.34 \\
fully trained & \textbf{74.94} & \textbf{35.54} & \textbf{38.52} & \textbf{44.61} \\
\hline
\end{tabular}
}
\setlength\belowcaptionskip{-2ex}
\captionsetup{font=small}
\caption{Predicate branch training comparison. ``ImageNet init'' means initializing the predicate CNN with ImageNet weights; ``entity detector'' means using the fixed conv\_body\_det features for predicates; ``fully trained'' means a separate CNN is initialized by the entity detector and fine-tuned end-to-end during training.}
% ``obj transform'' means using the lateral connected layers as the predicate feature extractor.}
\label{tab:abl_prd}
\end{table}
